A MIP-Based Approach for Multi-Robot Geometric Task-and-Motion Planning

We address multi-robot geometric task-and-motion planning (MR-GTAMP) problems in synchronous, monotone setups. The goal of the MR-GTAMP problem is to move objects with multiple robots to goal regions in the presence of other movable objects. To perform the tasks successfully and effectively, the robots have to adopt intelligent collaboration strategies, i.e., decide which robot should move which objects to which positions, and perform collaborative actions, such as handovers. To endow robots with these collaboration capabilities, we propose to first collect occlusion and reachability information for each robot as well as information about whether two robots can perform a handover action by calling motion-planning algorithms. We then propose a method that uses the collected information to build a graph structure which captures the precedence of the manipulations of different objects and supports the implementation of a mixed-integer program to guide the search for highly effective collaborative task-and-motion plans. The search process for collaborative task-and-motion plans is based on a Monte-Carlo Tree Search (MCTS) exploration strategy to achieve exploration-exploitation balance. We evaluate our framework in two challenging GTAMP domains and show that it can generate high-quality task-and-motion plans with respect to the planning time, the resulting plan length and the number of objects moved compared to two state-of-the-art baselines.

==> figures/all_results.tex <==
\begin{table*}[ht]
    \centering
    \scriptsize
\begin{minipage}[t]{0.48\linewidth}\centering
\caption{The parameters 1}
% \begin{tabular}{ c c }
% \toprule
% parameters  &  value \\
% \midrule
% Rated value &  1.5MW\\
% time & 50 s     \\
% value 1 & 100    \\
% value 2 & 200  \\
% value 3 & 300  \\
% value 4 & 400 \\
% value 5 & 500  \\
% value 6 & 600 \\
% VALUE 7 & 700 \\
% \bottomrule
% \end{tabular}

\begin{tabular}{lllllll}
    
    % \hline
    % Problem & \multicolumn{3}{c}{Success rate \%} & \multicolumn{3}{c}{Av. planning time} & \multicolumn{3}{c}{Av. makespan} & 
    % \multicolumn{3}{c}{Av. number of moved objects}\\
    % \cline{1-2}

    \hline
    % \multirow{2}{*}{Multirow} &  \multicolumn{3}{c}{Success rate \%} \\
    % \cline{2-4}
    % & PDDLStream & SimpleMRSC & Ours
    \\ [-1em]
    Prob. & \multicolumn{3}{c}{Success rate \%} & \multicolumn{3}{c}{Av. makespan} \\
    \\ [-1em]
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
    & Ap1 & Ap2 & Ours & Ap1 & Ap2 & Ours  \\
    \\ [-1em]
    \hline
    \\ [-1em]
    PA5 & 100.0 & 90.0 & \textbf{100.0} & 3.1 ($\pm$0.2) & 2.8 ($\pm$0.2) & \textbf{2.8 ($\pm$0.1)}  \\
    \\ [-1em]
    PA7 & 90.0 & 70.0 & \textbf{100.0} & 3.9 ($\pm$0.3) & 3.4 ($\pm$0.3) & \textbf{3.2 ($\pm$0.3)}  \\
    \\ [-1em]
    PA10 & 50.0 & 20.0 & \textbf{95.0} & 4.8 ($\pm$0.6) & N/A & \textbf{4.8 ($\pm$0.3)} \\
    \\ [-1em]
    BO8 & 70.0 & N/A & \textbf{95.0} & 4.6 ($\pm$0.1) & N/A & \textbf{3.5 ($\pm$0.3)} \\

    \hline 
    \\ [-1em]
    Prob. & \multicolumn{3}{c}{Av. planning time(s)} & \multicolumn{3}{c}{Av. motion cost} \\
    \\ [-1em]
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
    & Ap1 & Ap2 & Ours & Ap1 & Ap2 & Ours  \\
    \\ [-1em]
    \hline 
    \\ [-1em]
    PA5 & 5.5 ($\pm$0.8) & 4.0 ($\pm$0.7) & \textbf{2.3 ($\pm$0.4)} & 3.9 ($\pm$0.2) & \textbf{3.4 ($\pm$0.2)} & 3.5($\pm$0.2)  \\
    \\ [-1em]
    PA7 & 41.0 ($\pm$11.4) & 8.7 ($\pm$1.6) & \textbf{5.1 ($\pm$0.8)} & 5.2 ($\pm$0.3) & \textbf{4.0 ($\pm$0.3)} & 4.3 ($\pm$0.3)  \\
    \\ [-1em]
    PA10 & 388.5 ($\pm$134.3) & N/A & \textbf{17.5 ($\pm$5.5)} & \textbf{5.5 ($\pm$0.6)} & N/A & 5.6 ($\pm$0.4) \\
    \\ [-1em]
    BO8 &  466.8 ($\pm$91.0) & N/A & \textbf{104.3 ($\pm$14.6)} & 7.2 ($\pm$0.2) & N/A & \textbf{3.5 ($\pm$0.3)} \\

    \hline 
\end{tabular}


\end{minipage}\hfill%
\begin{minipage}[t]{0.48\linewidth}\centering
\caption{The parameters 2}
\label{tab:The parameters 2 }
\begin{tabular}{lllllllll}
    % \hline
    % Problem & \multicolumn{3}{c}{Success rate \%} & \multicolumn{3}{c}{Av. planning time} & \multicolumn{3}{c}{Av. makespan} & 
    % \multicolumn{3}{c}{Av. number of moved objects}\\
    % \cline{1-2}

    \hline
    % \multirow{2}{*}{Multirow} &  \multicolumn{3}{c}{Success rate \%} \\
    % \cline{2-4}
    % & PDDLStream & SimpleMRSC & Ours
    \\ [-1em]
    Problem & \multicolumn{2}{c}{Success rate \%} & \multicolumn{2}{c}{Av. planning time(s)} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
    \\ [-1em]
    2 robots & & 40.0 & & 117.8 ($\pm$31.6) & \\
    \\ [-1em]
    3 robots & & 100.0 & & 45.3 ($\pm$7.2) & \\
    \\ [-1em]
    4 robots & & 90.0 & & 189.7 ($\pm$101.9) & \\
    \\[-1em]
    & \multicolumn{2}{c}{Av. makespan} & \multicolumn{2}{c}{Av. motion cost}\\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
    \\ [-1em]
    2 robots & & 6.5 ($\pm$0.3) & & 9.0 ($\pm$0.4) &\\
    \\ [-1em]
    3 robots & & 5.1 ($\pm$0.3) & & 8.0 ($\pm$0.4) & \\
    \\ [-1em]
    4 robots & & 5.0 ($\pm$0.3) & & 8.1 ($\pm$0.5) &\\
    \\[-1em]
    % \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
    % & Ap1 & Ap2 & Ours & Ap1 & Ap2 & Ours & Ap1 & Ap2 & Ours & Ap1 & Ap2 & Ours \\
    % \\ [-1em]
    % \hline
    % \\ [-1em]
    % Clutter 15 & 100 & 100 & 100 & 216.1 & 39.9 & 31.9 & 3 & 2.7 & 2.7 & 3.7 & 4 & 3.7 \\
    % \\ [-1em]
    % Clutter 18 & 33 & 100 & 100 & 393.4 & 121.6 & 42.4 & 3 & 4.7 & 3 & 4 & 6.7 & 3.7 \\
    % \\ [-1em]
    % Clutter 21 & 0 & 40 & 100 & NA & 764 & 194.6 & NA & 6 & 3.2 & NA & 9 & 5 \\
    % \\ [-1em]
    \hline 
\end{tabular}
\end{minipage}
\end{table*}

==> figures/big_exp.tex <==
\begin{table*}[ht]\centering
\caption{Comparison of the proposed method with two different approaches. Ap1 presented in~\cite{garrett2020pddlstream}, Ap2 presented in~\cite{stilman2007manipulation}.}
\begin{tabular}{lllllllllllll}
    % \hline
    % Problem & \multicolumn{3}{c}{Success rate \%} & \multicolumn{3}{c}{Av. planning time} & \multicolumn{3}{c}{Av. makespan} & 
    % \multicolumn{3}{c}{Av. number of moved objects}\\
    % \cline{1-2}

    \hline
    % \multirow{2}{*}{Multirow} &  \multicolumn{3}{c}{Success rate \%} \\
    % \cline{2-4}
    % & PDDLStream & SimpleMRSC & Ours
    \\ [-1em]
    Problem & \multicolumn{3}{c}{Success rate \%} & \multicolumn{3}{c}{Av. planning time} & \multicolumn{3}{c}{Av. makespan} & \multicolumn{3}{c}{Av. motion cost}\\
    \\ [-1em]
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
    & Ap1 & Ap2 & Ours & Ap1 & Ap2 & Ours & Ap1 & Ap2 & Ours & Ap1 & Ap2 & Ours \\
    \\ [-1em]
    \hline
    \\ [-1em]
    Clutter 5 & 50 & 100 & 100 & 154.1 & 39.9 & 26.0 & 2.6 & 2.7 & 2.3 & 3.4 & 4.0 & 3.3 \\
    \\ [-1em]
    Clutter 7 & 30 & 100 & 100 & 243.1 & 121.6 & 33.0 & 2.3 & 4.7 & 3.5 & 3.3 & 6.7 & 4.1 \\
    \\ [-1em]
    Clutter 10 & 0 & 40 & 90 & N/A & 556.8 & 65.2 & N/A & 6.3 & 3.7 & N/A & 8.3 & 4.1 \\
    \\ [-1em]
    \hline 
\end{tabular}
% \end{center}
\label{tab:exp}
\end{table*}

==> figures/ds_example.tex <==
\begin{figure}[!t]
% Always try to place the figure on top of a column to save space
\centering
% Use linewidth to adjust width
% Use textheight(the total height of the column of text) to adjust height
%\includegraphics[width=\linewidth]{figs/XXX.jpg}
\includegraphics[width=0.9\linewidth]{figs/table_setting.png}
%\framebox[\linewidth]{\raisebox{0pt}[\linewidth][0pt]{{\LARGE The wow figure.}}}
\caption{An example dinner table setting task. The red blocks represent the plastic cups, the gray block represents a glass cup and the blue rectangles represent the goal regions.}
\label{fig:ds_example}
\end{figure}

==> figures/execution_seq.tex <==
\begin{figure*}[t!]
\centering

\begin{subfigure}[b]{\linewidth}
\centering
\includegraphics[width=.9\linewidth]{figs/pr2_seq_high.pdf}
\caption{An example execution trajectory of two robots in the box moving domain.\linebreak}
\end{subfigure}

\begin{subfigure}[b]{\linewidth}
\centering
\includegraphics[width=.9\linewidth]{figs/jaco_seq_high.pdf}
\caption{An example execution trajectory of two robots in the packaging domain.}
\end{subfigure}

\caption{The example scenes and execution trajectories of the domains we use to evaluate the proposed framework.}
\label{fig:scenes}

\end{figure*}

==> figures/exp_planning_time.tex <==
\begin{table*}[ht]\centering
\scriptsize
\caption{Comparison of the proposed method with two baseline methods in the two benchmark domains regarding the success rate, planning time, makespan and motion cost. The numbers in the problem names indicate the numbers of the included objects. We omit the solution quality results for Ap2 on PA10 because it has significantly lower success rate than other two methods.}
\begin{tabular}{lllllll}
    
    % \hline
    % Problem & \multicolumn{3}{c}{Success rate \%} & \multicolumn{3}{c}{Av. planning time} & \multicolumn{3}{c}{Av. makespan} & 
    % \multicolumn{3}{c}{Av. number of moved objects}\\
    % \cline{1-2}

    \hline
    % \multirow{2}{*}{Multirow} &  \multicolumn{3}{c}{Success rate \%} \\
    % \cline{2-4}
    % & PDDLStream & SimpleMRSC & Ours
    \\ [-1em]
    Prob. & \multicolumn{3}{c}{Success rate \%} & \multicolumn{3}{c}{Av. makespan} \\
    \\ [-1em]
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
    & Ap1 & Ap2 & Ours & Ap1 & Ap2 & Ours  \\
    \\ [-1em]
    \hline
    \\ [-1em]
    PA5 & 100.0 & 90.0 & \textbf{100.0} & 3.1 ($\pm$0.2) & 2.8 ($\pm$0.2) & \textbf{2.8 ($\pm$0.1)}  \\
    \\ [-1em]
    PA7 & 90.0 & 70.0 & \textbf{100.0} & 3.9 ($\pm$0.3) & 3.4 ($\pm$0.3) & \textbf{3.2 ($\pm$0.3)}  \\
    \\ [-1em]
    PA10 & 50.0 & 20.0 & \textbf{95.0} & 4.8 ($\pm$0.6) & N/A & \textbf{4.8 ($\pm$0.3)} \\
    \\ [-1em]
    BO8 & 70.0 & N/A & \textbf{95.0} & 4.6 ($\pm$0.1) & N/A & \textbf{3.5 ($\pm$0.3)} \\

    \hline 
    \\ [-1em]
    Prob. & \multicolumn{3}{c}{Av. planning time(s)} & \multicolumn{3}{c}{Av. motion cost} \\
    \\ [-1em]
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
    & Ap1 & Ap2 & Ours & Ap1 & Ap2 & Ours  \\
    \\ [-1em]
    \hline 
    \\ [-1em]
    PA5 & 5.5 ($\pm$0.8) & 4.0 ($\pm$0.7) & \textbf{2.3 ($\pm$0.4)} & 3.9 ($\pm$0.2) & \textbf{3.4 ($\pm$0.2)} & 3.5($\pm$0.2)  \\
    \\ [-1em]
    PA7 & 41.0 ($\pm$11.4) & 8.7 ($\pm$1.6) & \textbf{5.1 ($\pm$0.8)} & 5.2 ($\pm$0.3) & \textbf{4.0 ($\pm$0.3)} & 4.3 ($\pm$0.3)  \\
    \\ [-1em]
    PA10 & 388.5 ($\pm$134.3) & N/A & \textbf{17.5 ($\pm$5.5)} & \textbf{5.5 ($\pm$0.6)} & N/A & 5.6 ($\pm$0.4) \\
    \\ [-1em]
    BO8 &  466.8 ($\pm$91.0) & N/A & \textbf{104.3 ($\pm$14.6)} & 7.2 ($\pm$0.2) & N/A & \textbf{3.5 ($\pm$0.3)} \\

    \hline 
\end{tabular}
% \end{center}
\label{tab:exp_time}
\end{table*}

==> figures/exp_quality.tex <==
\begin{table}[ht]\centering
\caption{Comparison of the proposed method with two baseline methods in the two benchmark domains regarding the solution quality.}
\begin{tabular}{lllllll}
    % \hline
    % Problem & \multicolumn{3}{c}{Success rate \%} & \multicolumn{3}{c}{Av. planning time} & \multicolumn{3}{c}{Av. makespan} & 
    % \multicolumn{3}{c}{Av. number of moved objects}\\
    % \cline{1-2}

    \hline
    % \multirow{2}{*}{Multirow} &  \multicolumn{3}{c}{Success rate \%} \\
    % \cline{2-4}
    % & PDDLStream & SimpleMRSC & Ours
    \\ [-1em]
    Problem & \multicolumn{3}{c}{Av. makespan} & \multicolumn{3}{c}{Av. motion cost} \\
    \\ [-1em]
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
    & Ap1 & Ap2 & Ours & Ap1 & Ap2 & Ours  \\
    \\ [-1em]
    \hline
    \\ [-1em]
    Clutter 5 (D$1$) & 3.1 & 2.8 & 2.9 & 32.7 & 31.8 & 30.7  \\
    \\ [-1em]
    Clutter 7 (D$1$) & 3.5 & 3.2 & 3.4 & 38.6 & 34.1 & 34.6  \\
    \\ [-1em]
    Clutter 10 (D$1$) & N/A & 3.4 & 4.3 & N/A & 34.6 & 44.0 \\
    \\ [-1em]
    Clutter 5 (D$2$) & 3.0 & 1.1 & 2.1 & 58.0 & 35.8 & 33.1 \\
    \\ [-1em]
    Clutter 7 (D$2$) & 4.5 & 1.5 & 2.4 & 99.3 & 30.3 & 34.4 \\
    % Clutter 15 & 0 & 0 & 100 & N/A & N/A & 147.7 & N/A & N/A & 2.8 & N/A & N/A & 5.0 \\
    % \\ [-1em]
    % Clutter 18 & 0 & 0 & 100 & N/A & N/A & 663.5 & N/A & N/A & 3.2 & N/A & N/A & 6.4 \\
    % \\ [-1em]
    % Clutter 21 & 0 & 0 & 80 & N/A & N/A & 470.9 & N/A & N/A & 3.5 & N/A & N/A & 5.3 \\
    \hline 
\end{tabular}
% \end{center}
\label{tab:exp_quality}
\end{table}

==> figures/large.tex <==
\begin{table}[ht]
\caption{Our method can scale up to large problem instances containing $15$ to $21$ objects and $3$ to $4$ robots.}
\begin{tabular}{lllllllll}
    % \hline
    % Problem & \multicolumn{3}{c}{Success rate \%} & \multicolumn{3}{c}{Av. planning time} & \multicolumn{3}{c}{Av. makespan} & 
    % \multicolumn{3}{c}{Av. number of moved objects}\\
    % \cline{1-2}

    \hline
    % \multirow{2}{*}{Multirow} &  \multicolumn{3}{c}{Success rate \%} \\
    % \cline{2-4}
    % & PDDLStream & SimpleMRSC & Ours
    \\ [-1em]
    Problem & \multicolumn{2}{c}{Success rate \%} & \multicolumn{2}{c}{Av. planning time} & \multicolumn{2}{c}{Av. makespan} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
    \\ [-1em]
    Clutter 15 & & 100 & & 147.7 & 2.8 \\
    \\ [-1em]
    Clutter 18 & & 100 & & 663.5 & 3.2 \\
    \\ [-1em]
    Clutter 21 & & 80 & & 470.9 & 3.5 \\
    \\[-1em]
    % \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
    % & Ap1 & Ap2 & Ours & Ap1 & Ap2 & Ours & Ap1 & Ap2 & Ours & Ap1 & Ap2 & Ours \\
    % \\ [-1em]
    % \hline
    % \\ [-1em]
    % Clutter 15 & 100 & 100 & 100 & 216.1 & 39.9 & 31.9 & 3 & 2.7 & 2.7 & 3.7 & 4 & 3.7 \\
    % \\ [-1em]
    % Clutter 18 & 33 & 100 & 100 & 393.4 & 121.6 & 42.4 & 3 & 4.7 & 3 & 4 & 6.7 & 3.7 \\
    % \\ [-1em]
    % Clutter 21 & 0 & 40 & 100 & NA & 764 & 194.6 & NA & 6 & 3.2 & NA & 9 & 5 \\
    % \\ [-1em]
    \hline 
\end{tabular}
% \end{center}
\label{tab:large}
\end{table}

==> figures/scalability.tex <==
\begin{table}[ht]\centering
\scriptsize
\caption{Our method can scale up to large problem instances containing $18$ objects and $2$ to $4$ robots.}
\begin{tabular}{lllllllll}
    % \hline
    % Problem & \multicolumn{3}{c}{Success rate \%} & \multicolumn{3}{c}{Av. planning time} & \multicolumn{3}{c}{Av. makespan} & 
    % \multicolumn{3}{c}{Av. number of moved objects}\\
    % \cline{1-2}

    \hline
    % \multirow{2}{*}{Multirow} &  \multicolumn{3}{c}{Success rate \%} \\
    % \cline{2-4}
    % & PDDLStream & SimpleMRSC & Ours
    \\ [-1em]
    Problem & \multicolumn{2}{c}{Success rate \%} & \multicolumn{2}{c}{Av. planning time(s)} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
    \\ [-1em]
    2 robots & & 40.0 & & 117.8 ($\pm$31.6) & \\
    \\ [-1em]
    3 robots & & 100.0 & & 45.3 ($\pm$7.2) & \\
    \\ [-1em]
    4 robots & & 90.0 & & 189.7 ($\pm$101.9) & \\
    \\[-1em]
    & \multicolumn{2}{c}{Av. makespan} & \multicolumn{2}{c}{Av. motion cost}\\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
    \\ [-1em]
    2 robots & & 6.5 ($\pm$0.3) & & 9.0 ($\pm$0.4) &\\
    \\ [-1em]
    3 robots & & 5.1 ($\pm$0.3) & & 8.0 ($\pm$0.4) & \\
    \\ [-1em]
    4 robots & & 5.0 ($\pm$0.3) & & 8.1 ($\pm$0.5) &\\
    \\[-1em]
    % \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
    % & Ap1 & Ap2 & Ours & Ap1 & Ap2 & Ours & Ap1 & Ap2 & Ours & Ap1 & Ap2 & Ours \\
    % \\ [-1em]
    % \hline
    % \\ [-1em]
    % Clutter 15 & 100 & 100 & 100 & 216.1 & 39.9 & 31.9 & 3 & 2.7 & 2.7 & 3.7 & 4 & 3.7 \\
    % \\ [-1em]
    % Clutter 18 & 33 & 100 & 100 & 393.4 & 121.6 & 42.4 & 3 & 4.7 & 3 & 4 & 6.7 & 3.7 \\
    % \\ [-1em]
    % Clutter 21 & 0 & 40 & 100 & NA & 764 & 194.6 & NA & 6 & 3.2 & NA & 9 & 5 \\
    % \\ [-1em]
    \hline 
\end{tabular}
% \end{center}
\label{tab:scale}
\end{table}

==> figures/scenes.tex <==
\begin{figure*}[t!]
\centering
\begin{subfigure}[b]{\linewidth}\centering
\begin{tabular}{ccc}\centering
{\includegraphics[width=.25\linewidth,height=2.6cm]{figs/5.png}}\null\hfill&
{\includegraphics[width=.25\linewidth,height=2.6cm]{figs/7.png}}\null\hfill&
{\includegraphics[width=.25\linewidth,height=2.6cm]{figs/10.png}}
\end{tabular}
% \caption{The woman is holding the chopping board for the girl to cut the meat.}
\end{subfigure}

\caption{Three example scenes of Clutter 5, Clutter 7, Clutter 10 problems. There are $2$ robot arms and $3$ colored blocks. The goal is to move the colored blocks to the corresponding colored bins. The red region is the start region. To make the problems nontrivial, we constrain the white blocks can only be relocated inside the red region.}
\label{fig:scenes}

\end{figure*}

==> pmgrs.tex <==
\begin{algorithm}
\snnote{remove for now}
\caption{PMGRS($p, O_M^G$)}\label{alg:pmgrs}
% \caption{PMGRS($p, O_M^G, W, \mathbf{P}, \mathbf{M}, O_C, V_F, O_F, N_{smpl}, N_{mp}$)}\label{alg:pmgrs}
\begin{algorithmic}[1]
\WHILE {$\neg budget\_reached$}
% initialize a priority queue
\STATE {$queue = \text{PriorityQueue()}$}
% build the CMTG from the goal set and preds
\STATE {$\mathbf{C}^0 = \textsc{BuildCMTG}(O_M^G, p)$}
% \STATE {$p = $}
% \STATE {\textbf{initialize} $MG$}
% \STATE {$p = $\textbf{encode\_state}($W$)}
% \STATE {\textsc{BuildMG}(${\mathbf{M}, MG, \mathcal{A}, p, O_M}$)}
% get a set of plans 
\STATE {$\mathbf{AP} = $\textsc{ApproxPlan($\mathbf{C}^0$)}}
% push each AP into the queue
\FOR {$AP \in \mathbf{AP}$}
% we need to add required information to AP for exploration
\STATE {$AP.O_C = O_M$}
\STATE {$AP.\mathbf{M} = \{M \mid M \in O_M, M $ will be moved$\}$}
\STATE {$AP.V_F = \emptyset$}
\STATE {$AP.O_M^G = O_M^G$}
\STATE {$queue.add(AP, AP.length, AP.length)$}
\ENDFOR
% pop the elements in the queue one by one
\WHILE {$\neg queue.empty$}
\STATE {$AP = queue.pop()$}
% now try to explore AP
% get the last action
\STATE {$a = AP.last$}
\STATE {$a.M = $ objects that will be moved}
% sample the continuous parameters
\STATE {$k = SMPLCONT(a, AP.V_F, AP.O_C \setminus AP.\mathbf{M})$}
\STATE {$k.M = $ objects in $AP.M$ that collide with $k$}
% if k can't be found, we relax the constraint
\IF {$k$ is $\emptyset$}
\STATE {$k = SMPLCONT(a, AP.V_F, \emptyset)$}
\STATE {$k.M = $ objects in $AP.O_C$ that collide with $k$}
\ENDIF 
\IF {$k$ is $\emptyset$}
\STATE {\textbf{continue}}
\ENDIF
% else get new AP to explore
% update future volumes
\STATE {$\hat{V}_F = AP.V_F + k$}
% update the to move objects
\STATE {$\hat{O}_M^G = (AP.O_M^G \setminus a.M) \cup k.M)$}
\IF {$\hat{O}_M^G = \emptyset$}
\RETURN $\hat{V}_F$
\ENDIF
% update the current movable objects
\STATE {$\hat{O}_C = AP.O_C \setminus a.M$}
% now we can create new plans 
\STATE {$\hat{\mathbf{C}} = \textsc{BuildCMTG}(\hat{O}_M^G, p)$}
% create new aps
\STATE {$\hat{\mathbf{AP}} = \textsc{ApproxPlan}(\hat{\mathbf{C}})$}
\FOR {$\hat{AP} \in \hat{\mathbf{AP}}$}
\STATE {$\hat{AP}.O_C = \hat{O}_C$}
\STATE {$\hat{AP}.\mathbf{M} = \{M \mid M \in \hat{AP}.O_C, M\}$ will be moved}
\STATE {$\hat{AP}.V_F = \hat{V}_F$}
\STATE {$\hat{AP}.O_M^G = \hat{O}_M^G$}
\STATE {$queue.add(AP, \hat{AP}.V_F.length + \hat{AP}.length, \hat{AP}.length)$}
\ENDFOR 
\ENDWHILE
\RETURN {$\emptyset$}
\ENDWHILE
\RETURN {$\emptyset$}
\end{algorithmic}
\end{algorithm}
